GANSeg: Learning to Segment by Unsupervised Hierarchical Image Generation

Segmenting an image into its parts is a frequent preprocess for high-level vision tasks such as image editing. However, annotating masks for supervised training is expensive. Weakly-supervised and unsupervised methods exist, but they depend on the comparison of pairs of images, such as from multi-views, frames of videos, and image augmentation, which limits their applicability. To address this, we propose a GAN-based approach that generates images conditioned on latent masks, thereby alleviating full or weak annotations required in previous approaches. We show that such mask-conditioned image generation can be learned faithfully when conditioning the masks in a hierarchical manner on latent keypoints that define the position of parts explicitly. Without requiring supervision of masks or points, this strategy increases robustness to viewpoint and object positions changes. It also lets us generate image-mask pairs for training a segmentation network, which outperforms the state-of-the-art unsupervised segmentation methods on established benchmarks.

==> tex/ethics.tex <==
\section{Ethics} 
\textbf{Risks.} A GAN can be abused for creating deep fakes. However, our method does not work towards editing nor improved image quality but scene understanding. Our final output is a detector, which can not be abused to generate new images but unwanted surveillance applications are a risk.
\textbf{Benefits.} Since our method is entirely unsupervised, it could be applied on objects, animals, or situations that have not yet been labeled. 

==> tex/future_plan.tex <==
\cite{kulkarni2019canonical} propose to generate dense corresponding mapping via geometric cycle consistency. It maps pixels to a pre-defined template. It needs supervision on the silhouettes and a well-shaped template mesh of the same category.

\cite{kanazawa2018learning} propose a weak supervised 3D reconstruction method, which requires keypoints and silhouettes. It deforms a template mesh.

\cite{li2020self} propose a silhouettes-supervised single-view 3D reconstruction via semantic consistency. It also requires an off-the-shelf part segmentation method to start with, though the part segmentation method can be unsupervised and can be improved once trained end-to-end.



\paragraph{Possible idea.}
\begin{enumerate}
    \item use 3D keypoints. Use known rotation range. Use soft occlusion for Gaussian heatmaps.
    \item use 3D keypoints. Use known rotation range. Use perspective transformation to generate masks.
    \item extend the current mask generation with the 3D reconstruction \citep{\cite{li2020self}}. The 3D reconstruction works as a section instead of the main goal.
    \item use the NeRF to do segmentation. It takes positional encoding as input and output the mask (one-hot encoding using softmax). We have a learn constant embedding (or dynamical ones like LatentKeypointGAN) for each mask. We take the weighted sum as the embedding for that location. The concentration loss is on the final image, or we can render the mask out and enforce the concentration loss on the rendered mask.
    \item canonical surface mapping: map pixels to a position and then to another pixel by implicit function.
    \item insight argument: different form of representation can provide regularization on each other so they are more consistent.
\end{enumerate}
